OpenLLM-RTL: Open Dataset and Benchmark for LLM-Aided Design RTL Generation

The automated generation of design RTL based on large language model (LLM) and natural language instructions has demonstrated great potential in agile circuit design. However, the lack of datasets and benchmarks in the public domain prevents the development and fair evaluation of LLM solutions. This paper highlights our latest advances in open datasets and benchmarks from three perspectives: (1) RTLLM 2.0, an updated benchmark assessing LLM's capability in design RTL generation. The benchmark is augmented to 50 hand-crafted designs. Each design provides the design description, test cases, and a correct RTL code. (2) AssertEval, an open-source benchmark assessing the LLM's assertion generation capabilities for RTL verification. The benchmark includes 18 designs, each providing specification, signal definition, and correct RTL code. (3) RTLCoder-Data, an extended open-source dataset with 80K instruction-code data samples. Moreover, we propose a new verification-based method to verify the functionality correctness of training data samples. Based on this technique, we further release a dataset with 7K verified high-quality samples. These three studies are integrated into one framework, providing off-the-shelf support for the development and evaluation of LLMs for RTL code generation and verification. Finally, extensive experiments indicate that LLM performance can be boosted by enlarging the training dataset, improving data quality, and improving the training scheme.

==> section/deleted_content.tex <==




\iffalse

\iffalse
\iffalse
Achieving timing closure is of paramount importance in the VLSI design process. The Register-Transfer Level (RTL) stage not only lays the foundational blueprint by translating specifications into functional descriptions but also sets the tone for subsequent physical implementations. 
% As the design progresses into the later physical design phase, less space remains for further timing optimization. Thus, it's essential for RTL designers to intervene in timing issues, otherwise, significant delays and extended design cycles would be introduced. 
With limited scope for timing optimization in the later phases, it becomes imperative for RTL designers to actively address timing concerns to avoid delays and prolonged design cycles. 
Traditionally, timing slack analysis occurs only after the logic synthesis, focusing on the gate-level netlist. However, the growing complexity of modern integrated circuits and the rising costs of design iterations underscore the necessity for early left-shift timing slack analysis at the RTL stage.
\fi

Recent studies have witnessed an increasing integration of machine learning (ML) techniques into both timing optimization and early-stage timing evaluation. The post-synthesis optimization works mainly exploit the gate sizing technique, performing either reinforcement learning (RL)-based turn-around optimization~\cite{lu2021rl} or deep learning (DL)-based predictive optimization~\cite{nath2022transsizer}. During the logic design and synthesis stage, the timing optimization is achieved by tuning the flow~\cite{xie2020fist, liang2021flowtuner}, without the insights from RTL designs. 
\fi

In recent decades, machine learning has found extensive application in early-stage timing prediction, as listed in Table.~\ref{tbl:method}. During the post-synthesis stages, previous works all rely on the endpoint slack analysis from static timing analysis (STA). When the target stage netlist remains the same as in the current stage, precise timing predictions can be achieved by exploring suitable ML models and physical features based on timing paths~\cite{xie2022preplacement, he2022accurate, guo2022timing, barboza2019machine}. When the netlist is restructured during the design process (e.g., timing optimization), restructured information at each endpoint should be captured to provide the restructure-tolerant timing prediction flow~\cite{wang2023restructure}.
% leveraging timing-related physical data of the gate-level netlist or layout. 
% These works can be classified into two categories: netlist-invariant and netlist-restructured. In the netlist-invariant works~\cite{xie2022preplacement, he2022accurate, guo2022timing, barboza2019machine}, the target stage netlist remains the same as in the current stage. By exploring suitable ML models and physical features, precise timing predictions can be achieved. On the other hand, when the netlist is restructured during the design process (e.g., timing optimization), inaccuracy will be introduced into the timing prediction. To tackle this problem, ~\cite{wang2023restructure} captures the restructured information at each endpoint by integrating both netlist and layout information via multimodal fusion, and provides the restructure-tolerant timing prediction flow. 


At the RTL stage, limited works have been proposed until the last two years, and efforts have emerged to predict coarse-grained timing, either the worst negative slack (WNS) and total negative slack (TNS) of the sequential circuits or the max delay for the combinational modules. All these works bridge the RTL-netlist gap by exploiting various RTL representations (e.g., abstract syntax tree (AST) ~\cite{xu2022sns, sengupta2022good}, simple-operator graph~\cite{fang2023masterrtl}, and-inverter graph~\cite{ouyang2023asap}, or other types of directed acyclic graph~\cite{lopera2022applying}). Most recently, two works propose to evaluate the fine-grained timing paths at the RTL stage. ~\cite{lopera2023using} use graph neural network (GNN) to estimate the arrival time of the combinational blocks and ~\cite{sengupta2023early} employ multiclass classification to evaluate the delays of timing critical paths.
\fi




%\yao{These two unsolved challenges make most post-synthesis solutions~\cite{kahng2018using, barboza2019machine, guo2022timing, cao2022tf, wang2023restructure, he2022accurate, xie2022preplacement} inapplicable.}


% (1) No delay-related cell/net information is directly available. As a result, classical STA engines cannot handle it at all. (2) There is no direct mapping between most RTL signals and post-synthesis cells/nets, where delay labels are supposed to be annotated. (3) Design RTL is in code format, which cannot be processed directly. 


% we introduce RTL-Timer, an RTL stage endpoint timing slack monitoring and optimization framework.
% This framework provides fine-grained slack values and relative rank level predictions for all signals in RTL along with coarse-grained worst negative slack (WNS) and total negative slack (TNS). By enabling cross-design endpoint predictions for various RTL designs, the framework facilitates further timing optimization, benefitting both RTL designers and subsequent physical implementations using EDA tools. Our contributions are highlighted as follows:

% For instance, ~\cite{fang2023masterrtl} predicts WNS and TNS based on the bit-level simple operator graph representation and multi-stage timing modeling.~\cite{xu2022sns} samples RTL paths to provide WNS via a transformer model and an aggregation multilayer perceptron.~\cite{sengupta2022good} converts RTL into a register-driven tree, exploring various ML methods for TNS prediction. Other works~\cite{ouyang2023asap, lopera2022applying, wu2022lostin} concentrate on the combinational components of RTL designs and predict the delay. 
% Despite the fast RTL-stage timing modeling, these works yield coarse-grained design-level timing predictions, thereby lacking detailed predictive insights into RTL signals and offering limited optimization benefits to designers.



% During the post-synthesis stages, static timing analysis (STA) leveraging timing-related physical data from the gate-level netlist or layout can provide the accurate endpoint (EP) timing slack analysis. In recent decades, machine learning has found extensive application in accurately predicting timing slack in later stages, incorporating the current stage netlist or layout information combined with the STA result. 

% For example, ~\cite{xie2021net2} identifies the timing critical paths based on the net length at the synthesized netlist using a customized graph neural network.~\cite{wang2023restructure} achieved highly precise post-routing timing predictions through the fusion of a Graph Neural Network on the placed netlist and a Convolutional Neural Network on the layout image. Other studies also proposed precise endpoint slack prediction methods by exploring suitable ML models and features~\cite{he2022accurate, guo2022timing, barboza2019machine}. 


% However, these well-established models cannot be directly applied to RTL stage endpoint slack prediction, primarily due to their reliance on gate-level netlists and related physical information.

% and are naturally correlated with the target netlist timing slack.
%GBA-PBA


% At the RTL stage, different from the netlist with physical information, the RTL representation consists of the circuit functionality only. Over the past two years, efforts have emerged to predict coarse-grained worst negative slack (WNS) and total negative slack (TNS) at the design level. For instance, ~\cite{fang2023masterrtl} predicts WNS and TNS based on the bit-level simple operator graph representation and multi-stage timing modeling.~\cite{xu2022sns} samples RTL paths to provide WNS via a transformer model and an aggregation multilayer perceptron.~\cite{sengupta2022good} converts RTL into a register-driven tree, exploring various ML methods for TNS prediction. Other works~\cite{ouyang2023asap, lopera2022applying, wu2022lostin} concentrate on the combinational components of RTL designs and predict the delay. 
% Despite the fast RTL-stage timing modeling, these works yield coarse-grained design-level timing predictions, thereby lacking detailed predictive insights into RTL signals and offering limited optimization benefits to designers.



% Due to the absence of timing-related physical information in the RTL representation compared to netlists, and the mismatching endpoints between bit-wise netlists and signal-wise RTL, predicting endpoint slack becomes notably more challenging at the RTL stage. 

% To address these challenges, we introduce RTL-Timer, an RTL stage endpoint timing slack monitoring and optimization framework.
% This framework provides fine-grained slack values and relative rank level predictions for all signals in RTL along with coarse-grained worst negative slack (WNS) and total negative slack (TNS). By enabling cross-design endpoint predictions for various RTL designs, the framework facilitates further timing optimization, benefitting both RTL designers and subsequent design processes using EDA tools. Our contributions are highlighted as follows:



However, none of these works achieve the fine-grained timing evaluation for arbitrary sequential RTL designs, which makes the RTL stage timing prediction cannot offer further optimization benefits to the design process. We found that the RTL-stage timing paths (i.e. start-end register pair) collection process in~\cite{sengupta2023early} relies on the post-placement STA timing report, which makes the method unable to be generalized to new unseen designs. Here we summarize two key bottleneck factors that make the RTL-stage fine-grained modeling hard to achieve: (1) there are no direct mapping relations between the RTL code and the gate-level netlist, since RTL consists of single-bit or multi-bit signals and logic operators, while netlist is only made up with single-bit flip-flops and logic gates. (2) Different from the netlist or layout with physical information, the RTL representation consists of the circuit functionality only.

\iffalse
By adopting the simple-operator graph (SOG) for RTL modeling in ~\cite{fang2023masterrtl}, the registers in the bit-level SOG representation are one-to-one mapped to those in the netlist. However, the ML models used in the RTL stage are too coarse to capture the pattern from each register. Due to the second reason, the well-established post-synthesis models still cannot be directly transferred to the RTL stage fine-grained evaluation. 
\fi




To address these challenges, instead of persisting in the prediction of precise start-end register pair, we only focus on the arrival time of the timing path endpoint register, similar to the propagation mechanism in STA. We first extend the SOG representation into a general RTL representation that enables us to comprehensively examine the RTL design and supports pseudo-STA to provide reference timing-related physical information. Then we propose a fine-grained endpoint timing prediction flow for any RTL designs. We customize the loss function to comprehensively capture the hierarchical features of RTL design: from the entire design level to the driven cone of each endpoint and the timing paths inside the cone. Then the predictions from distinct representation variants are aggregated by the ensemble learning technique. By applying suitable ML models, both the arrival time and relative critical level of each endpoint are evaluated. 
The prediction framework facilitates further timing optimization, benefiting both RTL designers and subsequent physical implementations using EDA tools. Our contributions are highlighted as follows:



% \item To the best of our knowledge, we are the first to provide the fine-grained RTL stage endpoint timing prediction flow, integrated with predictive timing optimization strategies, named as RTL-Timer.
%enabling the predictive timing optimization strategies. 
%Evaluation across diverse RTL designs 

% Based on the fine-grained timing, the coarse-grained WNS and TNS prediction results outperform the state-of-the-art solutions. 

% \item We advance the state-of-the-art understanding of RTL code, utilizing various ML-friendly RTL representations to enable pseudo-STA at the RTL stage. The representations support the further ML models and can be aggregated by ensemble learning technique.

\item We advance the state-of-the-art understanding of RTL code by utilizing machine learning-friendly representations, facilitating pseudo-STA at the RTL stage. Four variances of the proposed representation support subsequent machine learning models and benefit from ensemble learning techniques.

    
\item Customized loss function is integrated into ML models to capture the influence of each endpoint's input cone. We explore various regression and learning-to-rank models for precise fine-grained register timing modeling.

    % \item We utilize ensemble learning techniques to aggregate bit-wise predictions from four IR-Netlists, employing regression and learning-to-rank models for RTL register signals.

\item Leveraging the predictions, we annotate register timing into RTL code to guide designers and select predictive timing optimization strategies from logic synthesis tools, resulting in up to 33.5\% improvement in TNS (avg. 9.9\%) and 16.4\% in WNS (avg. 3.1\%) with negligible impact on power and area and persisting through layout stages.


% we annotate the register timing into RTL code for designers and choose predictive timing optimization solutions from the logic synthesis tool to enhance timing quality. We achieve up to 33.5\% TNS (avg. 9.9\%) and 16.4\% WNS (avg. 3.1\%) improvements with negligible power and area overhead during the logic synthesis process, which still remain in the subsequent layout stages. 

    % \item Evaluation across diverse RTL designs demonstrates the generalizability and effectiveness of our techniques.


==> section/table_bak.tex <==
\section{Experimental Results} \label{sec:exper}
\subsection{Experimental Setup}
We implement our models using Scikit-learn framework. We train and evaluate our model on 21 open-source RTL designs by using 10-fold cross-validation. The benchmark covers all mainstream hardware description languages (HDLs), such as Verilog, VHDL, System Verilog, Chisel, and SpinalHDL and it also has a wide design scale range from 2K to 510K gates. 


\subsection{Evaluation Metrics}
To comprehensively evaluate our model, we employ three metrics: correlation coefficient (R), Mean Absolute Error Percentage (MAPE), and the average critical level coverage (COVR), defined as follows:
\begin{equation*}
\text{MAPE}= \dfrac{1}{n}\sum_{i=1}^{n}\dfrac{|y_i-\hat{y_i}|}{y_i} \times 100\%, \ \
\text{COVR}= \dfrac{1}{m}\sum_{g=1}^{m}\dfrac{\#.S_g \cap \#.\hat{S_g}}{\#.S_g} \times 100\%
\end{equation*}
The $\bar{\hat{y}}$ and $\bar{y}$ represent the average of predicted and measured values, respectively. The $g$ in COVR is the number of groups divided as the critical levels, in our work, we divide all the signal-wise endpoints into 4 groups, which are top 5\% as group1, 5\%-40\% as group2, 40\%-70\% as group3 and the rest as group4. For each group, we calculate the coverage of the number of intersections between the ground-truth group set $S_g$ and the predicted group set $\hat{S_g}$ among the ground-truth. 

These metrics bring a comprehensive and fair evaluation of ML models, where the higher correlation R and lower MAPE indicate better regression accuracy, and the higher coverage COVR represents a better ranking result.

\subsection{Modeling and Optimization Results}
% 1. Bitwise regression (four IR), compared with baseline MasterRTL
% 2. signal-wise + optimization
% 3. Design-wise, compared with MasterRTL and 2 solutions

\begin{figure*}
  \centering
  \includegraphics[width=0.95\linewidth]{fig/box.pdf}
  \caption{Box.}%Reducing training paths leads to decreasing model accuracy. Generated RTL designs mitigate the downward trend.}
  \label{fig:box}
  \vspace{-.1in}
\end{figure*}




\begin{figure*}
  \centering
  \includegraphics[width=0.95\linewidth]{fig/scatter.pdf}
  \caption{Scatter Plot.}%Reducing training paths leads to decreasing model accuracy. Generated RTL designs mitigate the downward trend.}
  \label{fig:scatter}
  \vspace{-.1in}
\end{figure*}


For the bit-wise arrival time modeling, based on the hierarchical features listed above, we exploit the XGBoost model with 100 estimation trees and a maximum depth of 45 for the regression task. For the paths of each endpoint, we use the most critical path from STA and $K$ sampled paths, where $K$ is decided by the following formula:

$K = ...$

The smoothing max operation is implemented with ....
Compared with the bit-wise path model used in~\cite{}, four IR-Netlist models all significantly outperform the baseline method. The SOG method can provide the best arrival time prediction among the four representations, and the others perform similarly. 

For the signal-wise modeling, we compare the calculated output from the four bit-wise models and the signal-wise regression model that ensembles all the predictions as model features, shown in Fig.~\ref{fig:box}(b). The model is XGBoost with 80 estimation trees and 30 maximum depth. By ensemble of all the predictions, the accuracy will be further improved. 
For the ranking result, by leveraging the pair-wise LTR model LambdaMART, the ranking result COVR is much better than the original regressions of four representations and the ensemble model. 

The experimental result of the signal-wise prediction and predictive optimization for each benchmark design is shown in Tabel.~\ref{tbl:result}. To further visualize the results, Fig.~\ref{fig:scatter} illustrates the original STA, bit-wise prediction, calculated signal-wise, and the prediction from ensemble learning of each endpoint arrival time on an example design \texttt{b18_1}. We summarize our observations below: 
\begin{itemize}
\item Our signal-wise regression and ranking models provides high accuracy predictions with average correlation R = 0.87, MAPE = 15\%, and COVR=80\% with low variance across the different design types.
\item Based on the predicted ranking, the predictive optimization can achieve timing optimization on both WNS and TNS on most designs, while maintaining or even decreasing the other design quality metrics (total area and power). 
\item Compared with the optimization with ground-truth ranking, our results are similar or even better.

\end{itemize}




\subsection{Ablation Study}

\subsection{Runtime Analysis}
Table.~\ref{tbl:runtime}

\begin{table}[h]
  \centering
  \renewcommand{\arraystretch}{1.1}
  \resizebox{0.45\textwidth}{!}{
    \begin{tabular}{c|c||c}
    \toprule
    \multicolumn{2}{
    c||}{\textbf{Stage}}   & \textbf{Runtime$^\star$}      \\
    \hline
    \hline
    \multirow{2}{*}{RTL preprocess} & IR-Netlist construction & 3.2\% \\ \cline{2-3}
    & IR-Netlist STA & 0.8\% \\
    % \multicolumn{2}{|c||}{SOG Construction}      & 3.4               \\
    \hline
    ML Feature extraction & Hierarchical modeling  & 0.1\%               \\
    \hline
    \multicolumn{2}{c||}{Prediction inference time}      & \textless{}0.001\% \\
    \hline \hline
    \multicolumn{2}{c||}{DC w. predictive optimization}      & 145\%
    \\
    \bottomrule 
    \end{tabular}
    }
    \begin{tablenotes}\scriptsize
        \item $^\star$ The runtime is presented as the proportion of logic synthesis runtime.
    \end{tablenotes}  
    \caption{MasterRTL Runtime Overhead.}  
        \label{tbl:runtime}
\end{table}


% \begin{table}[]
% \centering
% \begin{adjustbox}{width=0.45\textwidth}
% \begin{tabular}{c||cccc||c}
% \toprule
% \multirow{2}{*}{\textbf{Metrics}} & \multicolumn{4}{c||}{\textbf{Bitwise Modeling (ours)}}                             & \textbf{MasterRTL} \\ 
%                          & \multicolumn{1}{c|}{SOG}  & \multicolumn{1}{c|}{AIG}  & \multicolumn{1}{c|}{AIMG} & XAG  & SOG                  \\ \hline \hline
% R                        & \multicolumn{1}{c|}{0.85} & \multicolumn{1}{c|}{0.75} & \multicolumn{1}{c|}{0.76} & 0.77 & 0.1                  \\ 
% MAPE (\%)                 & \multicolumn{1}{c|}{11}   & \multicolumn{1}{c|}{13}   & \multicolumn{1}{c|}{15}   & 13   & 53                   \\ 
% COVR (\%)                 & \multicolumn{1}{c|}{65}   & \multicolumn{1}{c|}{71}   & \multicolumn{1}{c|}{71}   & 72   & 46                   \\ 
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \caption{}
% \label{tbl:result2}
% \end{table}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\setlength\tabcolsep{1pt}

\begin{table}[]
\begin{adjustbox}{width=0.49\textwidth}
\begin{tabular}{l||ccc||cccc||cccc}
\toprule
\multirow{2}{*}{\textbf{Design (\#.gates)}}  & \multicolumn{3}{c||}{\textbf{Singal-wise Prediction}} & \multicolumn{4}{c||}{\textbf{Opt. with Prediction (\%)}} & \multicolumn{4}{c}{\textbf{Opt. with Ground-truth (\%)}} \\
       & R                 & MAPE (\%)       & COVR (\%)    & WNS          & TNS          & Total Power      & Total Area      & WNS            & TNS             & Total Power         & Total Area        \\ \hline \hline
systemcdes(2k)   & 0.94              & 26             & 94              & \cellcolor{lightgreen}-1.3         & \cellcolor{lightgreen}-17          & \cellcolor{lightgreen}-0.8             & \cellcolor{lightgreen}1.8             & \cellcolor{lightgreen}-1.8           & \cellcolor{lightgreen}-17.3           & \cellcolor{lightgreen}0                   & \cellcolor{lightgreen}2.6               \\
systemcaes(5k)   & 0.86              & 23             & 77              & \cellcolor{lightgreen}-1.3         & \cellcolor{lightgreen}-13.7        & \cellcolor{lightgreen}2.1              & \cellcolor{lightgreen}3.2             & \cellcolor{lightgreen}-0.1           & \cellcolor{lightgreen}-14.4           & \cellcolor{lightgreen}2.1                 & \cellcolor{lightgreen}3.5               \\
VexRiscv1(7k)    & 0.87              & 24             & 86              & \cellcolor{lightred}6.9       & \cellcolor{lightred}7         & \cellcolor{lightred}-3.1          & \cellcolor{lightred}-2.8         & \cellcolor{lightgreen}-0.3           & \cellcolor{lightgreen}-1.1            & \cellcolor{lightgreen}0.5                 & \cellcolor{lightgreen}-0.8              \\
b29k)          & 0.91              & 7              & 86              & \cellcolor{lightred}5.6       & \cellcolor{lightred}-4.3      & \cellcolor{lightred}26.2          & \cellcolor{lightred}25           & \cellcolor{lightred}0.2         & \cellcolor{lightred}-6.6         & \cellcolor{lightred}26.2             & \cellcolor{lightred}23.4           \\
VexRiscv2(12k)   & 0.86              & 16             & 83              & \cellcolor{lightgreen}-0.2         & \cellcolor{lightgreen}-1.6         & \cellcolor{lightgreen}-0.9             & \cellcolor{lightgreen}0               & \cellcolor{lightgreen}-0.7           & \cellcolor{lightgreen}-1.8            & \cellcolor{lightgreen}-0.6                & \cellcolor{lightgreen}0.3               \\
VexRiscv3(12k)   & 0.83              & 30             & 86              & \cellcolor{lightgreen}-2.8         & \cellcolor{lightgreen}-4.8         & \cellcolor{lightgreen}3.9              & \cellcolor{lightgreen}1.2             & \cellcolor{lightgreen}-0.1           & \cellcolor{lightgreen}-2.2            & \cellcolor{lightgreen}1.9                 & \cellcolor{lightgreen}1                 \\
b22(13k)         & 0.74              & 18             & 83              & \cellcolor{lightred}0.7      & \cellcolor{lightred}-4.8      & \cellcolor{lightred}23.4          & \cellcolor{lightred}23.3         & \cellcolor{lightred}2.9         & \cellcolor{lightred}0.4          & \cellcolor{lightred}22.7             & \cellcolor{lightred}20.2           \\
b17(19k)         & 0.93              & 8              & 75              & \cellcolor{lightred}1.9       & \cellcolor{lightred}-5.2      & \cellcolor{lightred}2.2           & \cellcolor{lightred}0            & \cellcolor{lightgreen}-0.9           & \cellcolor{lightgreen}-5.6            & \cellcolor{lightgreen}0.2                 & \cellcolor{lightgreen}1                 \\
b17\_1(19k)      & 0.94              & 5              & 79              & \cellcolor{lightred}5.8       & \cellcolor{lightred}-3.2      & \cellcolor{lightred}1.7           & \cellcolor{lightred}2.1          & \cellcolor{lightred}0.9         & \cellcolor{lightred}-5.8         & \cellcolor{lightred}-0.6             & \cellcolor{lightred}0.4            \\
Rocket1(20k)     & 0.89              & 11             & 63              & \cellcolor{lightgreen}-7.1         & \cellcolor{lightgreen}-21.4        & \cellcolor{lightgreen}2.8              & \cellcolor{lightgreen}1.7             & \cellcolor{lightgreen}-3.7           & \cellcolor{lightgreen}-25.4           & \cellcolor{lightgreen}-66                 & \cellcolor{lightgreen}2.9               \\
Rocket2(29k)     & 0.9               & 18             & 64              & \cellcolor{lightgreen}-7           & \cellcolor{lightgreen}-23.1        & \cellcolor{lightgreen}-69.4            & \cellcolor{lightgreen}-0.6            & \cellcolor{lightgreen}-4.1           & \cellcolor{lightgreen}-23.1           & \cellcolor{lightgreen}1.6                 & \cellcolor{lightgreen}-0.8              \\
Rocket3(32k)     & 0.88              & 12             & 69              & \cellcolor{lightgreen}-7.2         & \cellcolor{lightgreen}-17.4        & \cellcolor{lightgreen}-69.4            & \cellcolor{lightgreen}-0.6            & \cellcolor{lightgreen}-6.2           & \cellcolor{lightgreen}-18.3           & \cellcolor{lightgreen}-69.7               & \cellcolor{lightgreen}0.8               \\
wb\_conmax(36k)  & 0.91              & 12             & 83              & \cellcolor{lightgreen}-1.9         & \cellcolor{lightgreen}-3           & \cellcolor{lightgreen}3.4              & \cellcolor{lightgreen}2.7             & \cellcolor{lightgreen}-0.9           & \cellcolor{lightgreen}-0.6            & \cellcolor{lightgreen}3                   & \cellcolor{lightgreen}2.1               \\
b18(45k)         & 0.76              & 13             & 84              & \cellcolor{lightgreen}-16.4        & \cellcolor{lightgreen}-33.5        & \cellcolor{lightgreen}3.8              & \cellcolor{lightgreen}3.9             & \cellcolor{lightgreen}-17.9          & \cellcolor{lightgreen}-35.5           & \cellcolor{lightgreen}3.6                 & \cellcolor{lightgreen}3.4               \\
b18\_1(45k)      & 0.88              & 10             & 86              & \cellcolor{lightgreen}-3.9         & \cellcolor{lightgreen}-26          & \cellcolor{lightgreen}0.5              & \cellcolor{lightgreen}-0.4            & \cellcolor{lightgreen}-9.8           & \cellcolor{lightgreen}-27             & \cellcolor{lightgreen}1.8                 & \cellcolor{lightgreen}0.2               \\
FPU(56k)         & 0.89              & 31             & 85              & \cellcolor{lightred}6.2       & \cellcolor{lightred}0.2       & \cellcolor{lightred}0.5           & \cellcolor{lightred}1            & \cellcolor{lightred}4.3         & \cellcolor{lightred}-1.7         & \cellcolor{lightred}-86.6            & \cellcolor{lightred}0.6            \\
MuraxFast(159k)  & 0.79              & 16             & 78              & \cellcolor{lightgreen}-1.7         & \cellcolor{lightgreen}-3           & \cellcolor{lightgreen}-0.1             & \cellcolor{lightgreen}-0.1            & \cellcolor{lightred}2.4         & \cellcolor{lightred}-2.2         & \cellcolor{lightred}0                & \cellcolor{lightred}-0.5           \\
VexRiscv4(220k)  & 0.77              & 16             & 67              & \cellcolor{lightgreen}-4.8         & \cellcolor{lightgreen}-18.6        & \cellcolor{lightgreen}0                & \cellcolor{lightgreen}-0.7            & \cellcolor{lightgreen}-7.2           & \cellcolor{lightgreen}-21.9           & \cellcolor{lightgreen}0.4                 & \cellcolor{lightgreen}-1                \\
VexRiscv5(459k)  & 0.92              & 4              & 81              & \cellcolor{lightgreen}-1.8         & \cellcolor{lightgreen}-4.6         & \cellcolor{lightgreen}0.2              & \cellcolor{lightgreen}-1.3            & \cellcolor{lightgreen}-3.6           & \cellcolor{lightgreen}-10.7           & \cellcolor{lightgreen}0.3                 & \cellcolor{lightgreen}-0.6              \\
VexRiscv6(496k)  & 0.9               & 6              & 82              & \cellcolor{lightgreen}-1.5         & \cellcolor{lightgreen}-12.8        & \cellcolor{lightgreen}0.4              & \cellcolor{lightgreen}-0.5            & \cellcolor{lightgreen}-3             & \cellcolor{lightgreen}-5.3            & \cellcolor{lightgreen}0.3                 & \cellcolor{lightgreen}-1.3              \\
VexRiscv7(510k)  & 0.87              & 6              & 81              & \cellcolor{lightgreen}-5.7         & \cellcolor{lightgreen}-7.2         & \cellcolor{lightgreen}0.5              & \cellcolor{lightgreen}-0.8            & \cellcolor{lightgreen}-3             & \cellcolor{lightgreen}-12.3           & \cellcolor{lightgreen}0.5                 & \cellcolor{lightgreen}-0.2              \\ \hline
\textbf{Average w. } & \multirow{2}{*}{\textbf{0.87}}     & \multirow{2}{*}{\textbf{15}}    & \multirow{2}{*}{\textbf{80}}  
&\textbf{-1.9}  &\textbf{-10.4} & \textbf{-3.4} & \textbf{2.8} & \textbf{-2.5} &\textbf{-11.2} &\textbf{-7.5} &\textbf{2.7} \\
\textbf{Average2} &     & & &

\textbf{-3.1}         & \textbf{-9.9}         & \textbf{-5.9}             & \textbf{0.5}             & \textbf{-3}             & \textbf{-10.6}           & \textbf{-5.7}                & \textbf{0.6}
\\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{}
\label{tbl:result}
\end{table}


\begin{table}[]
\resizebox{0.495\textwidth}{!}{
\begin{tabular}{l||c|l|c|c|c}
\toprule
\textbf{} & \multicolumn{1}{c|}{\textbf{Benchmark}} & \textbf{Name}         & \textbf{\#Gates} & \textbf{\#Endpoints} & \multicolumn{1}{l}{\textbf{HDL Type}} \\
\hline
\hline
1     & \multirow{6}{*}{ITC'99~\cite{}}      
& b20          & 9K           & 430         & \multirow{6}{*}{VHDL}        \\
2     &                               & b22          & 13K          & 613         &                              \\
3     &                               & b17          & 19K          & 1324        &                              \\
4     &                               & b17\_1       & 19K          & 1311        &                              \\
5     &                               & b18          & 45K          & 925         &                              \\
6     &                               & b18\_1       & 45K          & 930         &                              \\ \cline{2-6}
7     & \multirow{4}{*}{OpenCores~\cite{}}    & systemcdes   & 2K           & 190         & \multirow{4}{*}{Verilog}     \\
8     &                               & systemcaes   & 5K           & 670         &                              \\
9     &                               & wb\_conmax   & 36K          & 770         &                              \\
10    &                               & FPU          & 56K          & 3825        &                              \\ \cline{2-6}
11    & \multirow{3}{*}{Chipyard~\cite{}}     & Rocket_1   & 20K          & 2569        & \multirow{3}{*}{Chisel}      \\
12    &                               & Rocket_2 & 29K          & 3916        &                              \\
13    &                               & Rocket_3       & 32K          & 4003        &                              \\ \cline{2-6}
14    & \multirow{8}{*}{VexRiscv~\cite{}}     & Vex\_1       & 7K           & 1299        & \multirow{8}{*}{SpinalHDL}   \\
15    &                               & Vex\_2       & 12K          & 1524        &                              \\
16    &                               & Vex\_3       & 12K          & 1440        &                              \\
17    &                               & MuraxFast    & 159K         & 68186       &                              \\
18    &                               & Vex\_4       & 220K         & 74677       &                              \\
19    &                               & Vex\_5       & 459K         & 146899      &                              \\
20    &                               & Vex\_6       & 496K         & 146905      &                              \\
21    &                               & Vex\_7       & 510K         & 146969      &       
\\
\bottomrule
\end{tabular}
}
\caption{}
\label{tab:my-table}
\end{table}


\begin{tabular}{c||c|c|c|l} \toprule
                                 & \multicolumn{1}{c|}{}                                   &                                         & \multicolumn{2}{c}{\textbf{General}}                  & \multicolumn{1}{|c}{}                                                                                                   \\ \cline{4-5} 
& \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{Method}}} & \multirow{-2}{*}{\textbf{Fine-Grained}} & \textbf{Sequential}       & \textbf{Cross-Design}     & \multicolumn{1}{c}{\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Applied in \\     Optimization\end{tabular}}}} \\ \hline \hline                       & ~\cite{xie2022preplacement, he2022accurate, guo2022timing, barboza2019machine, wang2023restructure}                                                       & \checkmark                                       & \checkmark                         & \checkmark                         &                                                                                                                        \\ \hline
                                 & ICCAD‘22~\cite{lopera2022applying}                                               &                                         &                           & \checkmark                         &                                                                                                                        \\
                                 & ISCA'22~\cite{xu2022sns}                                                &                                         & \checkmark                         & \checkmark                         &                                                                                                                        \\
                                 & ICCAD'22~\cite{sengupta2022good}                                               &                                         & \checkmark                         & \checkmark                         &                                                                                                                        \\
                                 & ICCAD'23~\cite{fang2023masterrtl}                                               &                                         & \checkmark                         & \checkmark                         &                                                                                                                        \\
                                 & MLCAD'23~\cite{ouyang2023asap}                                               &                                         &                           & \checkmark                         &                                                                                                                        \\
                                 & MLCAD'23~\cite{lopera2023using}                                               & \checkmark                                       &                           & \checkmark                         &                                                                                                                        \\
                                 & MLCAD'23~\cite{sengupta2023early}                                               & \checkmark                                       & \checkmark                         &                           & \multicolumn{1}{c}{\checkmark}                                                                                                  \\
\multirow{-8}{*}{\textbf{RTL}}            & \cellcolor[HTML]{C5D9F1}Ours                          & \cellcolor[HTML]{C5D9F1}\checkmark               & \cellcolor[HTML]{C5D9F1}\checkmark & \cellcolor[HTML]{C5D9F1}\checkmark & \multicolumn{1}{c}{\cellcolor[HTML]{C5D9F1}\checkmark}           \\ \bottomrule                                                  
\end{tabular}
